Bounded combinatorics and uniform models for hyperbolic 3-manifolds

Bounded-type 3-manifolds arise as combinatorially bounded gluings of irreducible 3-manifolds chosen from a finite list. We prove effective hyperbolization and effective rigidity for a broad class of 3-manifolds of bounded type and large gluing heights. Specifically, we show the existence and uniqueness of hyperbolic metrics on 3-manifolds of bounded type and large heights, and prove existence of a bilipschitz diffeomorphism to a combinatorial model described explicitly in terms of the list of irreducible manifolds, the topology of the identification, and the combinatorics of the gluing maps.

==> elcmacs.tex <==
%% Macros for ELT I and II.

%%%%%%   until I draw them, make figures blank:
%\long\def\brealfig#1#2#3{\blankfig{#1}{2in}{#3}}
\renewcommand{\segment}{\subsection*}

\newcommand{\T}{{\mathbf T}}
\newcommand{\inj}{\operatorname{inj}}
\newcommand{\pleat}{\operatorname{\mathbf{pleat}}}
\newcommand{\short}{\operatorname{\mathbf{short}}}
\newcommand{\vertices}{\operatorname{vert}}
\newcommand{\collar}{\operatorname{\mathbf{collar}}}
\newcommand{\bcollar}{\operatorname{\overline{\mathbf{collar}}}}
\newcommand{\good}{\operatorname{\mathbf{good}}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\carriedby}{\prec}
\newcommand{\subtrack}{<}
\newcommand{\strongly}{\carriedby\carriedby}
\newcommand{\I}{{\mathbf I}}
\newcommand{\tprec}{\prec_t}
\newcommand{\fprec}{\prec_f}
\newcommand{\bprec}{\prec_b}
\newcommand{\pprec}{\prec_p}
\newcommand{\ppreceq}{\preceq_p}
\newcommand{\sprec}{\prec_s}
\newcommand{\cpreceq}{\preceq_c}
\newcommand{\cprec}{\prec_c}
\newcommand{\topprec}{\prec_{\rm top}}
\newcommand{\Topprec}{\prec_{\rm TOP}}
\newcommand{\fsub}{\mathrel{\scriptstyle\searrow}}
\newcommand{\bsub}{\mathrel{\scriptstyle\swarrow}}
\newcommand{\fsubd}{\mathrel{{\scriptstyle\searrow}\kern-1ex^d\kern0.5ex}}
\newcommand{\bsubd}{\mathrel{{\scriptstyle\swarrow}\kern-1.6ex^d\kern0.8ex}}
%\newcommand{\fsubeq}{\mathrel{\genfrac{}{}{0pt}{}{\searrow}{\raise.1ex\hbox{=}}}}
\newcommand{\fsubeq}{\mathrel{\raise-.7ex\hbox{$\overset{\searrow}{=}$}}}
%\newcommand{\bsubeq}{\mathrel{\genfrac{}{}{0pt}{}{\swarrow}{\raise.1ex\hbox{=}}}}
\newcommand{\bsubeq}{\mathrel{\raise-.7ex\hbox{$\overset{\swarrow}{=}$}}}
\newcommand{\tw}{\operatorname{tw}}
\newcommand{\base}{\operatorname{base}}
\newcommand{\trans}{\operatorname{trans}}
\newcommand{\rest}{|_}
\newcommand{\bbar}{\overline}
\newcommand{\UML}{\operatorname{\UU\MM\LL}}
\newcommand{\EL}{\mathcal{EL}}
\newcommand{\tsum}{\sideset{}{'}\sum}
\newcommand{\tsh}[1]{\left\{\kern-.9ex\left\{#1\right\}\kern-.9ex\right\}}
\newcommand{\Tsh}[2]{\tsh{#2}_{#1}}
\newcommand{\qeq}{\mathrel{\approx}}
\newcommand{\Qeq}[1]{\mathrel{\approx_{#1}}}
\newcommand{\qle}{\lesssim}
\newcommand{\Qle}[1]{\mathrel{\lesssim_{#1}}}
\newcommand{\simp}{\operatorname{simp}}
\newcommand{\vsucc}{\operatorname{succ}}
\newcommand{\vpred}{\operatorname{pred}}
\newcommand\fhalf[1]{\overrightarrow {#1}}
\newcommand\bhalf[1]{\overleftarrow {#1}}
\newcommand\sleft{_{\text{left}}}
\newcommand\sright{_{\text{right}}}
\newcommand\sbtop{_{\text{top}}}
\newcommand\sbot{_{\text{bot}}}
\newcommand\sll{_{\mathbf l}}
\newcommand\srr{_{\mathbf r}}
\newcommand\Hleft{H\sleft}
\newcommand\Hright{H\sright}
\newcommand\geod{\operatorname{\mathbf g}}
%\newcommand\mtorus[1]{\FF(#1)}
\newcommand\mtorus[1]{\boundary U(#1)}
\newcommand\A{\mathbf A}
\newcommand\Aleft[1]{\A\sleft(#1)}
\newcommand\Aright[1]{\A\sright(#1)}
\newcommand\Atop[1]{\A\sbtop(#1)}
\newcommand\Abot[1]{\A\sbot(#1)}
\newcommand\boundvert{{\boundary_{||}}}
\newcommand\storus[1]{U(#1)}
\newcommand\Homega{\omega_H}
\newcommand\Momega{\omega_M}
\newcommand\nomega{\omega_\nu}
\newcommand\twist{\operatorname{tw}}
\newcommand\modl{M_\nu}
\newcommand\MT{{\mathbb T}}
\newcommand\Teich{{\mathcal T}}
\newcommand\parab{\operatorname{parab}}
\newcommand\bersfcn{\LL}
\newcommand\neck{\varepsilon}
\newcommand\epshrink{\ep_{T}}
\newcommand\shear{\operatorname{\mathbf{shear}}}

%%%%%% These are for CKGII:
\newcommand{\bp}{\operatorname{\rm bp}}
\newcommand{\bv}{\operatorname{\rm bv}}
\newcommand{\bg}{\operatorname{\rm bg}}
\newcommand{\slices}{\operatorname{\rm slices}}
\newcommand{\towall}{\mathrel{\dashv}}
\newcommand{\wallto}{\mathrel{\vdash}}
\newcommand{\wall}{\mathrel{|}}
\newcommand{\stprec}{\mathrel{\vee}}
\newcommand{\lands}{\operatorname{\YY}}
\newcommand\add[1]{{\langle #1 \rangle}}
\newcommand\thk[1]{{{\rm thick}(#1)}}

\newcommand\interior{{\rm int}}

